Top-k Combinatorial Bandits with Full-Bandit Feedback

Top-k Combinatorial Bandits generalize multi-armed bandits, where at each round any subset of $k$ out of $n$ arms may be chosen and the sum of the rewards is gained. We address the full-bandit feedback, in which the agent observes only the sum of rewards, in contrast to the semi-bandit feedback, in which the agent observes also the individual arms' rewards. We present the Combinatorial Successive Accepts and Rejects (CSAR) algorithm, which generalizes SAR (Bubeck et al, 2013) for top-k combinatorial bandits. Our main contribution is an efficient sampling scheme that uses Hadamard matrices in order to estimate accurately the individual arms' expected rewards. We discuss two variants of the algorithm, the first minimizes the sample complexity and the second minimizes the regret. We also prove a lower bound on sample complexity, which is tight for $k=O(1)$. Finally, we run experiments and show that our algorithm outperforms other methods.

==> acknowledgements.tex <==
\section*{Acknowledgements}
First and foremost, I would like to thank my supervisor Prof. Yishay Mansour for his dedication and collaboration. His endless availability and assistance are highly appreciated.\\
A special thank is granted to Nadav Merlis, for his helpful conversations and uncountable advices that helped me dive deeper into the field of Multi-Armed Bandits. I also thank Avishai Wagner who was always glad to think with me about interesting problems that came up as part of the research. \\
I thank my team at Intel, and especially my managers Nufar Gaspar and Jeremie Dreyfuss, for the interesting and inspiring conversations, for their support and understanding and their great willingness to help.\\
Kudos to my dear friends for their support along the way, especially Yossi Tamarov, Avi Caciularu and Or Perel. I will always appreciate their true friendship. I'd also like to thank my buddies Jonathan Shafer and Uri Meir, who accompanied me along the Masters and made this period unforgettable.\\
Finally, I’d like to take this opportunity to thank Prof. Naama Friedmann and the Adi Lautman interdisciplinary program for an amazing and inspiring academic experience.

==> csar.tex <==
\section{Combinatorial Successive Accepts and Rejects Algorithm}
In this chapter we present the Combinatorial Successive Accepts and Rejects Algorithm for top-k combinatorial bandits. We begin by presenting an efficient estimation algorithm that estimates the expected rewards for all the arms, and then discuss the main algorithm that uses the estimation algorithm in order to find the best subset of $k$ arms. Finally, we bound the sample complexity and regret achieved by the algorithm.

\subsection{Estimation Algorithm}
The first algorithm we discuss suggests an efficient method to estimate the expected rewards of the arms under full bandit feedback. The algorithm gets as inputs a set $\mathcal{N}$ of $n$ arms, a subset size $k$, a level of accuracy $\epsilon$, a level of confidence $\delta$, and two more dummy variables that will be used later on: a set of accepted arms $\mathcal{A}$ and a set of the top $2k$ arms $\mathcal{T}$. The algorithm first partitions $\mathcal{N}$ into sets of size $2k$. In each of those sets, it makes use of the Hadamard matrix as an instructor for the subsets to sample. Let $H$ be the Hadamard matrix of size $2k$, then for each row $H_i\,(i\ne 1)$ the algorithm partitions the arms according to the positive and negative entries in $H_i$. Since in every row exactly half of the entries are positive, the partition forms two sets of size $k$. For $i=1$, $H_1$ has only positive entries, so the algorithm partitions arbitrarily to two sets. Each of these sets is sampled enough times to get a good estimate on its expected reward. Then, the sets' estimated rewards are summed according to their sign in $H$. This way we get a vector $\hat{Z}$ that is equal in expectation to $H\theta$. Finally, to estimate the individual arms' rewards, the algorithm uses the Hadamard matrix inverse $H^{-1}\hat{Z}=\frac{1}{2k}H^\intercal\hat{Z}$, which is the least squares estimator for $\theta$ given $\hat{Z}$.


\begin{algorithm}
\caption{EST1$(\mathcal{N},k,\epsilon,\delta,\mathcal{A},\mathcal{T})$}
\label{alg:estimate}
$n=|\mathcal{N}|$;
$m(\epsilon,\delta)=\frac{2}{\epsilon^2}\log\frac{2n}{\delta}$\\
Partition $\mathcal{N}$ into sets of size $2k$: $\mathcal{N}_1\dots \mathcal{N}_\frac{n}{2k}$  \\
\For{$l=1\dots \frac{n}{2k}$}{
Let $\mathcal{N}_l=\{j_1\dots j_{2k}\}$\\
$S_{1,{-1}}=\{j_1,\dots ,j_k\},\,S_{1,{+1}}=\{j_{k+1},\dots ,j_{2k}\}$ \Comment{$i=1$}\\
$S_{i,{b}}=\{j\in\mathcal{N}_l\,|\,H_{ij}=b\}$ \Comment{$i=2\dots 2k,\, b\in\{-1,+1\}$}\\
\For{$i\in [2k],b\in\{-1,+1\}$}{
Sample $S_{i,b}$ for $m(\epsilon,\delta)$ times and observe rewards $r_1,\dots,r_m$\\
$\hat\mu_{i,b}=\frac{1}{m}\sum_{t} r_t$
}
$\hat{Z}_1=\hat\mu_{1,{+1}} + \hat\mu_{1,{-1}}$ \Comment{$i=1$}\\
$\hat{Z}_i=\hat\mu_{i,{+1}} - \hat\mu_{i,{-1}}$ \Comment{$i=2\dots 2k,\, b\in\{-1,+1\}$}

$\hat\theta_{\mathcal{N}_l}=\frac{1}{2k}H^\intercal \hat{Z}$
}
\Return $\hat\theta$
\end{algorithm}

\paragraph{Remark 1.} For simplicity, we assume that $2k$ divides $n$. Otherwise, when partitioning the arms in the first step we may repeat arms in the last subset. This increases the number of estimations by at most $2k$, and thus we replace $n$ with $n+2k$ in the number of samples $m(\epsilon,\delta)$. Since $n>2k$, this modification does not change the order of magnitude of the sample complexity and regret.

\paragraph{Remark 2.} We assume that there exists a Hadamard matrix of size $2k$. Otherwise, let $2q\in\mathbb{N}$ be a multiple of $2k$ such that there exists a Hadamard matrix of size $2q$. Partition the arms into subsets of size $2q$ (instead of $2k$), and then in each row the number of positive and negative entries is a multiple of $k$. Then, partition them to $\frac{q}{k}$ sets of size $k$, sample each one separately, and then sum them to get $\hat\mu_{+1}$ and $\hat\mu_{-1}$. This modification changes the sample complexity and regret by at most a constant factor.


\begin{lemma}\label{lemma:PACest1}
For any $\epsilon,\delta>0$ and any set of $n$ arms $\mathcal{N}$, EST1 returns an estimated reward vector $\hat\theta$ such that
\[Pr\Big[\forall i,\,|\hat\theta_i-\theta_i|\leq \epsilon\Big]\geq 1-\delta\]
\end{lemma}

\begin{proof}
We first prove that $\hat\theta$ is an unbiased estimator of the reward vector $\theta$. For simplicity we fix $N_1=\{1\dots 2k\}$ and write $\hat\theta$ instead of $\hat\theta_{N_1}$. 
First note that for each set $S$, the average $\hat\mu_S=\frac{1}{m}\sum_t r_t$ is an unbiased estimator for the set's reward, hence
\[\mathbb{E}[\hat\mu_S]=\mu_S=\sum_{i\in S} \theta_i\]
As a consequence for each $i\ne 1$, $\hat{Z}_i$ satisfies
\[\mathbb{E}[\hat{Z}_i]= \mu_{i,+1} - \mu_{i,-1} = \sum_{j\in S_{i,+1}} \theta_j - \sum_{j\in S_{i,-1}} \theta_j =\sum_{j=1}^{2k} H_{ij}\theta_j = H_i^\intercal\theta \]
and for $i=1$
\[\mathbb{E}[\hat{Z}_1]= \mu_{1,+1} + \mu_{1,-1} = \sum_{j\in S_{1,+1}} \theta_j + \sum_{j\in S_{1,-1}} \theta_j =\sum_{j=1}^{2k} H_{1j}\theta_j = H_1^\intercal\theta \]
Namely the vector $\hat{Z}$ satisfies $\mathbb{E}[\hat{Z}]=H\theta$. Finally,
\[\mathbb{E}[\hat\theta]=\frac{1}{2k}H^\intercal\mathbb{E}[\hat{Z}]=\frac{1}{2k}H^\intercal H\theta=\theta\]

We now prove the lemma. Fix some subset $S$ sampled by the algorithm, and we prove that the estimation noise $\hat\eta_S=\hat\mu_S-\mu_S$ is $\frac{k}{m}$-subgaussian. By definition,
\[\hat\mu_S=\frac{1}{m}\sum_{t=1}^m r_t= \frac{1}{m}\sum_{t=1}^m \sum_{i\in S} X_i= \frac{1}{m}\sum_{t=1}^m \sum_{i\in S} (\theta_i + \eta_{it})=\mu_S+\frac{1}{m}\sum_{t=1}^m \sum_{i\in S} \eta_{it}\]
Since the noise terms $\eta_{it}$ are 1-subgaussians, and we sum over $k$ such terms in each $t$, the total estimation noise is also subgaussian with parameter $\frac{k}{m}$. Accordingly, the estimation noise of each $\hat{Z}_i$, which is given by $\eta_{Z_i}=\hat{Z}_i-\mathbb{E}[\hat{Z}_i]=\eta_{i,+1}-\eta_{i,-1}$ is $\frac{2k}{m}$-subgaussian (and the same for $i=1$). Finally, the estimation noise of $\hat\theta$ which is given by
\[\hat\theta_i-\theta_i=\frac{1}{2k}\sum_{j=1}^{2k} H_{ij}\eta_{Z_j} \]
is also subgaussian with parameter $\frac{2k}{2km}=\frac{1}{m}$. Thus,
\[Pr\Big[|\hat\theta_i-\mathbb{E}[\hat\theta_i]|\geq \epsilon\Big]\leq 2\exp\bigg({-\frac{\epsilon^2}{2} m}\bigg)=\frac{\delta}{n}\]
where in the last equality we substituted the number of samples $m(\epsilon,\delta)$. Finally, the probability of error in the estimation of one parameter is at most $\frac{\delta}{n}$, and thus by the union bound the probability of error in one parameter or more is at most $\delta$.

\end{proof}


\newpage
\subsection{Main Algorithm}
We now show how to use the estimation method described above to find the best subset. The algorithm, which we call \emph{Combinatorial Successive Accepts and Rejects} (CSAR), is based on SAR \cite{bubeck2013multiple} for multiple arms identification. CSAR works in phases. In each phase $t$ it maintains a decaying level of accuracy $\epsilon_t$ and confidence $\delta_t$ and uses EST1 to estimate the arms to a given level of accuracy and confidence. Then, it sorts the arms according to their estimations $\hat\theta^t_1\geq \hat\theta^t_2\geq\dots \geq\hat\theta^t_n$, and accepts arms whose estimated reward is bigger than $\hat\theta^t_{k+1}$ by at least $2\epsilon_t$, i.e., $\hat\theta^t_{i}- \hat\theta^t_{k+1}\geq 2\epsilon_t$, as they are optimal with high confidence. Similarly, it rejects arms whose estimated reward is smaller than $\hat\theta^t_{k}$ by at least $2\epsilon_t$. The algorithm proceeds until $n-k$ arms are rejected.

\begin{algorithm}
\caption{Combinatorial Successive Accepts and Rejects (CSAR)}
\label{alg:csar}
$\mathcal{N}^1=\mathcal{N}; \mathcal{A}^1=\emptyset$;
$\epsilon_1 = \frac{1}{2}; \delta_1 = \frac{6}{\pi^2}\delta$\\
\While{$|\mathcal{N}^t\cup\mathcal{A}^t|>k$}{
$\hat\theta^t= EST1(\mathcal{N}^t,k,\epsilon_t,\delta_t,\mathcal{A}^t,\mathcal{T}^t)$\\
Sort $\mathcal{N}^t\cup\mathcal{A}^t$ according to $\hat\theta^t$ such that $\hat\theta^t_1\geq \hat\theta^t_2\geq\dots \geq\hat\theta^t_n$ \\
$\mathcal{T}^t=\{1\dots 2k\}$\\
$\mathcal{A}=\{i\in \mathcal{N}_t\,|\,\hat\theta_i^t - \hat\theta^t_{k+1} > 2\epsilon_t\}$\\
$\mathcal{R}=\{i\in \mathcal{N}^t\,|\,\hat\theta^t_k - \hat\theta_i^t > 2\epsilon_t\}$\\
$\mathcal{A}^{t+1}=\mathcal{A}^t\cup\mathcal{A}$\\
$\mathcal{N}^{t+1}=\mathcal{N}^t\setminus(\mathcal{A}\cup\mathcal{R}) $ \\
$\epsilon_{t+1}=\frac{\epsilon_t}{2}; \delta_{t+1}=\frac{\delta_1}{t^2};t=t+1$
}
\Return{$\mathcal{A}_t\cup\mathcal{N}_t$}
\end{algorithm}

We now prove the correctness of CSAR, namely that it returns the best subset with high probability.
\begin{lemma}\label{thm:pac}
For any $\delta>0$, CSAR with EST1 is $(0,\delta)$-PAC, i.e., it finds the optimal subset with probability at least $1-\delta$.
\end{lemma}

\begin{proof}
For each phase $t$, define the event $E_t$ that one arm is estimated poorly, i.e.,
\[E_{t}=\{\exists i\,|\hat\theta_{t}^i-\theta_{t}^i|>\epsilon_t\}\]
and let $E=\bigcup_t E_t$. Note that the algorithm is wrong only if at some phase it rejected an optimal arm or accepted a sub-optimal arm. This might happen only under the event $E$. Hence, the probability that the algorithm is wrong is bounded by the probability of $E$.
By Lemma 1 we know that for any $t$, $Pr[E_t]\leq\delta_t$ and thus by the union bound
\[Pr[E]\leq\sum_t Pr[E_t]\leq \sum_t \delta_t= \sum_{t=1}^{T}\frac{\delta_1}{t^2}\leq \delta_1 \sum_{t=1}^{\infty} \frac{1}{t^2}=\frac{6}{\pi^2}\delta\cdot\frac{\pi^2}{6}=\delta\]
Accordingly, the algorithm returns the optimal subset with probability at least $1-\delta$.\\
For the rest of the proofs we assume that $E$ did not happen.
\end{proof}

\paragraph{Remark 3.} One can easily modify CSAR to be $(\epsilon,\delta)$-PAC. For that, we provide the algorithm also with a level of accuracy $\epsilon$, and instead of stopping only when $k$ arms are left, we may stop earlier when $\epsilon_t\leq \frac{\epsilon}{2k}$ and return the top $k$ arms according to the last estimation. It is not hard to show that the surviving arms are $2\epsilon_t$ close to the optimal arms and therefore the output is at most $k\epsilon_t=\epsilon$ far from the optimal subset. 
%In this case, the sample complexity is similar to (\ref{eq:sampleComp}), but replacing $\Delta_i$ with $\max\{\Delta_i,\frac{\epsilon}{2k}\}$ since the algorithm might stop earlier.


\subsection{Sample Complexity}
In this section, we bound CSAR's sample complexity in the following theorem.
\begin{theorem}\label{lemma:armSampleComp}
For any $\delta>0$, the total number of samples performed by CSAR with EST1 is at most
\begin{equation}\label{eq:sampleComp}
    M= O\bigg(\sum_{i=1}^n\Big(\frac{1}{\Delta_i^2}\log\frac{n}{\delta}+\log\log\frac{1}{\Delta_i}\Big)\bigg)
\end{equation}
\end{theorem}

Note that CSAR's sample complexity is comparable with the $O\big(\sum_{i=1}^n \frac{1}{\Delta_i^2}\log\frac{n}{\delta}\big)$ sample complexity of the original Successive Elimination algorithm for best arm identification \citep{even2006action}, and also with algorithms for multiple arms identification \citep{kalyanakrishnan2010efficient, kalyanakrishnan2012pac}, although in these models the agent samples one arm in each round and not $k$ like in the combinatorial model.

To bound the sample complexity, we break the proof into parts. We first prove the following lemma regarding the number of times each arm is sampled until it is accepted or rejected.
\begin{lemma_thm}\label{lemma:armSampleComp2}
For any arm $i$, let $T_i$ be the phase when $i$ is rejected (if it is sub-optimal) or accepted (if it is optimal), and let $M_i(\tau)$ be the number of times $i$ is sampled by CSAR up to phase $\tau$, then for each $\tau\leq T_i$
\[M_i(\tau)\leq Ck\cdot 4^{\tau}\big(\log\frac{2n}{\delta}+2\log \tau\big)\]
where $C$ is a constant.
\end{lemma_thm}


\begin{proof}
Let $i$ be an arm. In every phase $t<T_i$, arm $i$ is sampled as part of $2k\times 2$ subsets and each subset is sampled $m(\epsilon_t,\delta_t)$ times where $\epsilon_t=2^{-t}$ and $\delta_t=\frac{\delta_1}{t^2}$, thus we have
\begin{equation} 
\begin{split}
M_i(\tau) &= \sum_{t=1}^{\tau}4k m(\epsilon_t,\delta_t)=\sum_{t=1}^{\tau}\frac{8k}{\epsilon_t^2}\log\frac{2n}{\delta_t}= 8k\sum_{t=1}^{\tau}(2^{t})^2\log\frac{t^2 2n}{\delta_1}=\\
&=8k\Big(\sum_{t=1}^{\tau}4^{t}\log t^2+\log\frac{2n}{\delta_1}\sum_{t=1}^{\tau}4^{t}\Big)\leq
Ck\big(2\log \tau+\log\frac{2n}{\delta}\big)\cdot 4^{\tau}
\end{split}
\end{equation}
\end{proof}

We now use Lemma \ref{lemma:armSampleComp2} to bound the total number of times each arm is sampled.

\begin{lemma_thm}\label{lemma:armSampleComp}
For each arm $i\in[n]$, the number of times it is sampled until it is rejected (if it is sub-optimal) or accepted (if it is optimal) is bounded by
\[M_i \leq \frac{Ck}{\Delta_i^2}\big(\log\frac{2n}{\delta}+2\log\log\frac{1}{\Delta_i}\big)\]
\end{lemma_thm}

\begin{proof}
We analyze the case that $i$ is sub-optimal, but the analysis for optimal arms is similar. Let $i$ be a sub-optimal arm and denote by $T_i$ the phase it is rejected. \\
If $E$ did not happen then for any phase $t$ and any arm $i$ we have $|\hat\theta_i^t-\theta_i|\leq \epsilon_t$. That also implies that the difference between the real $k$th arm and the arm estimated to be in the $k$th place satisfies $|\hat\theta_k^t-\theta_k|\leq \epsilon_t$, since mixing the order of the arms can happen only between arms that are within the same $\epsilon_t$-neighborhood.
As long as $i$ was not rejected, i.e., $\forall t=1\dots T_i-1$, it holds that
\[2\epsilon_t\geq \hat\theta_k^t-\hat\theta_i^t\geq (\theta_k-\epsilon_t)-(\theta_i+\epsilon_t)=(\theta_k-\theta_i)-2\epsilon_t=\Delta_i-2\epsilon_t \]
Substituting $\epsilon_t=2^{-t}$ we get $\Delta_i\leq 4\epsilon_t=4\cdot 2^{-t}$.
This is true also for $t=T_i-1$, and thus we get $T_i\leq\log\frac{4}{\Delta_i}$. Substituting $T_i$ in Lemma \ref{lemma:armSampleComp2} yields the desired bound.
\end{proof}

Finally, we bound CSAR's sample complexity.
\begin{lemma_thm}
For any $\delta>0$, the total number of samples used by CSAR with EST1 is bounded by
\[M= O\bigg(\sum_{i=1}^n\Big(\frac{1}{\Delta_i^2}\log\frac{n}{\delta}+\log\log\frac{1}{\Delta_i}\Big)\bigg)\]
\end{lemma_thm}
\begin{proof}
Since each subset sampled by the algorithm consists of $k$ arms, the number of samples is equal to the number of arms sampled divided by $k$. In the worst case, each of the arms is sampled until it is accepted or rejected, hence
\[M\leq\frac{1}{k}\sum_{i=1}^n M_i=O\bigg(\sum_{i=1}^n \Big(\frac{1}{\Delta_i^2}\log\frac{n}{\delta}+\log\log\frac{1}{\Delta_i}\Big)\bigg) \]
where $M_i$ is given by Lemma \ref{lemma:armSampleComp}.
\end{proof}

To understand how this upper bound scales, consider the following rewards distribution $X_i\sim Ber(p_i)$ where
\[p_i=\begin{cases}
    \frac{1}{2}+\frac{\epsilon}{k} & i=1\dots k\\
    \frac{1}{2} & i=k+1\dots n\\
\end{cases}\]
In this case, for any arm $i=k+1\dots n$ it holds $\Delta_i=\frac{\epsilon}{k}$ and thus the number of samples is bounded by $M=O\big(\frac{nk^2}{\epsilon^2}\log\frac{n}{\delta}\big)$ (ignoring $\log \log$ terms).

\newpage
\subsection{Regret}
We now analyze the regret.
Notice that while CSAR aims to minimize the sample complexity, it does not minimize the regret. This is because at each time the algorithm chooses a subset, the regret it achieves is affected not only by the arms it selected, but also by the arms it did not select. In other words, the gap that should be considered is between the sub-optimal arm $i\in\{k+1\dots n\}$ that was actually selected and the optimal arm $j\in\{1 \dots k\}$ that would have been selected instead. We denote this gap by $\Delta_{j:i}=\theta_j-\theta_i$. Using this notation, we may bound the regret of the algorithm. 

\begin{theorem}\label{thm:weakRegret}
For any $n,k\leq\frac{n}{2}$ and time horizon $T>n$ the regret of CSAR with EST1 is at most
\[R=O\Bigg(\sum_{i=k+1}^n  \frac{\Delta_{1:i}}{\Delta_{k:i}^2} k\log T\Bigg)\]
\end{theorem}

\begin{proof}
Since only sub-optimal arms are responsible for regret, we consider only them. For any sub-optimal arm $i$, the maximal gap it may suffer is $\Delta_{1:i}$. Accordingly, the regret is bounded by
\[R\leq\sum_{i=k+1}^n M_i\Delta_{1:i}\leq O\Bigg(\sum_{i=k+1}^n  \frac{\Delta_{1:i}}{\Delta_{k:i}^2} k\log \frac{n}{\delta}\Bigg)\]
where we used the bound on $M_i$ from Lemma \ref{lemma:armSampleComp}, while neglecting $\log\log$ factors.\\
In order to translate this bound to terms of the time horizon $T$, recall that if the algorithm goes wrong, it might suffer a regret of $kT$, and this happens with probability $\delta$. To avoid it, we take $\delta=\frac{1}{kT}$ and thus we can write the upper bound above as 
\[R\leq O\Bigg(\sum_{i=k+1}^n  \frac{\Delta_{1:i}}{\Delta_{k:i}^2} k\log T \Bigg)\]
where we used the fact that $T>n>k$ to neglect these factors inside the $\log$.
\end{proof}

Note that this bound is tight for CSAR with EST1. For example, consider the following problem. Each arm $i\in [n]$ is associated with a Gaussian random variable $X_i\sim\mathcal{N}(\theta_i,1)$, where
\begin{equation}\label{instance:regret}
    \theta_i=\begin{cases}
    \Delta_{+} & i<k\\
    0 & i=k\\
    -\Delta_{-} & i>k
    \end{cases}
\end{equation}
and assume $\Delta_+ \gg \Delta_-$. On this problem, CSAR will accept the first $k-1$ arms after a small number of iterations. Then, for the rest of the run it will sample only arms with expected reward of at most $0$. In each call to EST1 each of the $n-k+1$ arms is sampled $\frac{8k}{\epsilon_t^2}\log\frac{n}{\delta_t}$ times, and it keeps being sampled until $2\epsilon_t<\Delta_{-}$. Therefore, the total regret of the algorithm is $\Theta \Big(\frac{\Delta_{+}}{\Delta_{-}^2}(n-k)k\log\frac{n}{\delta}\Big)$. In the following section we discuss a modification for the algorithm that helps achieve smaller regret.

\subsection{Modified algorithm with improved regret}
The reason for the $\Delta_{1:i}$ factors in Theorem \ref{thm:weakRegret} is due to the fact that when we identify an arm as optimal, we stop sampling it, and thus suffer regret for its absence. Instead, we consider the following modification for the algorithm in order to improve the regret. When we accept an arm, instead of preventing it from being sampled, we fix it. Namely, we sample it in every subset until the end of the run. This will assure that we suffer gaps such as $\Delta_{1:i}$ only for a small number of rounds. 

Accordingly, we modify the estimation algorithm to support fixed arms. Now, the algorithm gets as input also a set $\mathcal{A}$ of accepted arms that must be sampled in each subset. Instead of using the Hadamard matrix of size $2k$, it takes a smaller one of size $2k'$ where $k'=k-|\mathcal{A}|$ is the number of arms that can be sampled in each subset after keeping room for the fixed arms. Most of the algorithm remains the same, except for the need to have good estimations for the fixed arms' expected rewards. This is because it needs to eliminate those rewards from the sampled subsets and stay only with the arms that should be estimated. For that, we provide it with a set ${\mathcal{T}}$ of the top $2k$ arms, according to the last phase estimations, and run EST1 separately on them.


\begin{algorithm}
\caption{EST2$(\mathcal{N},k,\epsilon,\delta,\mathcal{A},\mathcal{T})$}
\label{alg:estimate-fixed}
$n=|\mathcal{N}|;\,k'=k-|\mathcal{A}|;\,m(\epsilon,\delta,k')=\frac{2k}{k'}\frac{2}{\epsilon^2}\log\frac{2n}{\delta}$\\
$\hat\theta_1\dots\hat\theta_{2k} = EST1({\mathcal{T}},\epsilon,\delta,\mathcal{A},\mathcal{T})$\\
Partition $\mathcal{N}$ into sets of size $2k'$: $\mathcal{N}_1\dots \mathcal{N}_\frac{n}{2k'}$  \\
\For{$l=1\dots \frac{n}{2k'}$}{
Let $\mathcal{N}_l=\{j_1\dots j_{2k'}\}$\\
$S'_{1,{-1}}=\{j_1,\dots ,j_{k'}\},\,S'_{1,{+1}}=\{j_{k'+1},\dots ,j_{2k'}\}$\Comment{$i=1$}\\
$S'_{i,{b}}=\{j\in\mathcal{N}_l\,|\,H_{ij}=b\}$ \Comment{$i=2\dots 2k',\, b\in\{-1,+1\}$}\\
\For{$i\in [2k'],b\in\{-1,+1\}$}{
$S_{i,b}=S_{i,b}'\cup\mathcal{A}$\\
Sample $S_{i,b}$ for $m(\epsilon,\delta)$ times and observe rewards $r_1,\dots,r_m$\\
$\hat\mu_{i,b}=\frac{1}{m}\sum_{t} r_t$
}
$\hat{Z}_1=\hat\mu_{1,+1} + \hat\mu_{1,-1} - 2\sum_{a\in\mathcal{A}} \hat\theta_a$ \Comment{$i=1$}\\
$\hat{Z}_i=\hat\mu_{i,{+1}} - \hat\mu_{i,{-1}}$ \Comment{$i=2\dots 2k',\, b\in\{-1,+1\}$}

$\hat\theta_{\mathcal{N}_l}=\frac{1}{2k'}H^\intercal \hat{Z}$
}
\Return $\hat\theta$
\end{algorithm}

We first prove the correctness of EST2.
\begin{lemma}
For any $\epsilon,\delta>0$ and any set of $n$ arms $\mathcal{N}$ and set of accepted arms $\mathcal{A}$, EST2 returns an estimated reward vector $\hat\theta$ such that
\[Pr\Big[\forall i,\,|\hat\theta_i-\theta_i|\leq \epsilon\Big]\geq 1-\delta\]
\end{lemma}

\begin{proof}
The proof is similar to Lemma \ref{lemma:PACest1}, so we only stress the differences.
First, when proving that $\hat\theta$ is an unbiased estimator of $\theta$, we have $S=S'\cup\mathcal{A}$, hence for each $i\neq 1$, $\hat{Z}_i$ satisfies
\[\begin{split}
    \mathbb{E}[\hat{Z}_i]= &\mu_{i,+1} - \mu_{i,-1} = \sum_{j\in S_{i,+1}'} \theta_j + \sum_{j\in \mathcal{A}} \theta_j - \bigg(\sum_{j\in S_{i,-1}'} \theta_j + \sum_{j\in \mathcal{A}} \theta_j \bigg) \\ =&\sum_{j\in S_{i,+1}'} \theta_j - \sum_{j\in S_{i,-1}'} \theta_j=\sum_{j=1}^{2k'} H_{ij}\theta_j = H_i^\intercal\theta
\end{split} \]
and for $i=1$
\[\begin{split}
    \mathbb{E}[\hat{Z}_1]=& \mu_{1,-1} + \mu_{1,+1} - 2\sum_{j\in\mathcal{A}} \theta_j \\ =&\sum_{j\in S_{1,+1}'} \theta_j + \sum_{j\in \mathcal{A}} \theta_j + \sum_{j\in S_{1,-1}'} \theta_j + \sum_{j\in \mathcal{A}} \theta_j - 2\sum_{j\in\mathcal{A}} \theta_j \\ =&\sum_{j\in S_{1,+1}'} \theta_j + \sum_{j\in S_{1,-1}'} \theta_j=\sum_{j=1}^{2k'} H_{1j}\theta_j = H_1^\intercal\theta
\end{split} \]

Second, we want to prove that each $\eta_{\hat{Z}_i}$ is subgaussian. For any $i\neq 1$ the proof remains the same, the only difference is for $i=1$, for which we have
\begin{equation}\label{eqn:Z1}
    \hat{Z}_1= \hat\mu_{1,-1} + \hat\mu_{1,+1} - 2\sum_{j\in\mathcal{A}} \hat\theta_j
\end{equation}
Thus the noise consists of $\eta_{1,-1}, \,\eta_{1,+1}$ which are $\frac{k}{m}$-subgaussians, and the noise of each $\hat\theta_j$. We proved in Lemma \ref{lemma:PACest1} that the latter is $\frac{1}{m}$-subgaussian, and therefore when summing at most $k$ such terms and multiplying by $2$ we get that the last term in (\ref{eqn:Z1}) is subgaussian with parameter at most $\frac{2k}{m}$. Summing all terms, we get that $\eta_{\hat{Z}_i}$ is subgaussian with parameter at most $\frac{4k}{m}$.

Finally, we recall that the estimation noise of $\hat\theta$ which is given by
\[\hat\theta_i-\theta_i=\frac{1}{2k'}\sum_{j=1}^{2k'} H_{ij}\eta_{Z_j} \]
and thus it is also subgaussian with parameter at most $\frac{4k}{2k'm}$. Thus for $m=\frac{2k}{k'}\frac{2}{\epsilon^2}\log\frac{2n}{\delta}$ we get
$Pr\Big[|\hat\theta_i-\mathbb{E}[\hat\theta_i]|\geq \epsilon\Big]\leq\frac{\delta}{n}$, and by the union bound the toal probability of error is at most $\delta$.
\end{proof}

Using EST2 instead of EST1 improves CSAR's regret, as shown in the following theorem.
\begin{theorem}\label{thm:regretUpperBound}
For any $n,k$ and time horizon $T>n$, the regret of CSAR with EST2 is at most
\begin{equation}\label{eqn:regret}
    R= O\Bigg(\bigg(\sum_{i=1}^k\frac{\Delta_{i:(k+i)}}{\Delta^2} + \sum_{i=k+1}^n  \frac{1}{\Delta_i} \bigg) k\log T \Bigg)
\end{equation}
\end{theorem}

Note that this is an improvement over CSAR with EST1. For example, on problem (\ref{instance:regret}), the first arms will be fixed after a small number of rounds and the regret will be
\[R=\Theta\bigg(\Big(k\frac{\Delta_+}{\Delta_-^2}+\frac{n-k}{\Delta_-}\Big)k\log T\bigg)\]
which is better than $\Theta \Big(\frac{\Delta_{+}}{\Delta_{-}^2}(n-k)k\log T\Big)$ as long as $\frac{\Delta_+}{\Delta_-}\gtrapprox 1+\frac{k}{n}$.


To prove the upper bound on the regret of CSAR with EST2, we first prove the following lemma that bounds the regret caused by each sub-optimal arm.

\begin{lemma_thm}\label{lemma:individualArmRegret}
For any sub-optimal arm $i$ with gap $\Delta_i$, its' contribution to the regret is bounded by
\[R_i\leq O\bigg(\frac{1}{\Delta_i}k\log\frac{n}{\delta}\bigg)\]
\end{lemma_thm}

\begin{proof}
Since all of the expressions in this proof depends on a factor of $Ck\log\frac{2n}{\delta}$, we omit it along the proof and multiply by it at the end.

Fix a sub-optimal arm $i$. By Lemma \ref{lemma:armSampleComp2}, the number of times $i$ is chosen up to phase $\tau\leq T_i$ is $M_i(\tau)\leq 4^\tau$ (up to $\log$ factors), and it is rejected by phase $T_i\leq\log\frac{4}{\Delta_i}$.
We split the optimal arms $\{1\dots k\}$ according to $\Delta_i$, and bound separately the regret $R_i^<$ caused by missing an optimal arm $j\in[k]$ with $\Delta_j\leq\Delta_i$, and the regret $R_i^>$ for the arms $j\in[k]$ with $\Delta_j>\Delta_i$.
\begin{itemize}
    \item For any $j\in[k]$ such that $\Delta_j\leq \Delta_i$, the maximal gap we pay for taking arm $i$ instead of arm $j$ is at most $\Delta_{j:i}\leq 2\Delta_i$, and thus the regret of such case is bounded by \[R_i^<\leq M_i(T_i)\Delta_{j:i}\leq \frac{1}{\Delta_i^2}\cdot (\Delta_j+\Delta_i)\leq \frac{1}{\Delta_i^2}\cdot 2\Delta_i= \frac{2}{\Delta_i}\]
    \item For any $j\in[k]$ such that $\Delta_j>\Delta_i$, arm $j$ is accepted at some point before arm $i$ is rejected, thus at some point we can be sure that arm $i$ is not played instead of arm $j$. Let $l=\arg\min_{j:\Delta_j>\Delta_i}\Delta_j$. We showed that each optimal arm $j$ is accepted at phase $T_j\leq\log\frac{4}{\Delta_i}$, thus we can write the regret of arm $i$ up to phase $T_j$ as
    \begin{equation*}
    \begin{split}
        R_i^>\leq &M_i(T_1)\Delta_{1:i}+ \big(M_i(T_2)-M_i(T_1)\big)\Delta_{2:i} + \dots + \big(M_i(T_l)-M_i(T_{l-1})\big)\Delta_{l:i}\\
        = & M_i(T_1)(\Delta_{1:i}-\Delta_{2:i}) + M_i(T_2)(\Delta_{2:i}-\Delta_{3:i}) + \dots + M_i(T_j)\Delta_{j:i} \\ = &\sum_{j=1}^{l-1} M_i(T_j) (\Delta_{j:i}-\Delta_{(j+1):i})+ M_i(T_l)\Delta_{l:i}
    \end{split}
    \end{equation*}
    We write $\Delta_{j:i}=\Delta_{j:(k+1)}+\Delta_{k:i}-\Delta_{k:(k+1)}=\Delta_{j}+\Delta_{i}-\Delta$ and substitute $M_i(T_j)\leq\frac{1}{\Delta_j^2}$ to get
    \begin{equation*}
        \begin{split}
        R_i^>\leq&\sum_{j=1}^{l-1} \frac{\Delta_{j}-\Delta_{j+1}}{\Delta_j^2} + \frac{\Delta_{l}+\Delta_i}{\Delta_l^2} \\
        \leq & \int_{\Delta_l}^{\Delta_1} \frac{1}{x^2}dx + \frac{2\Delta_{l}}{\Delta_l^2} \\ =&\bigg(\frac{1}{\Delta_l}-\frac{1}{\Delta_1}\bigg) +\frac{2}{\Delta_l}\leq \frac{3}{\Delta_l}\leq \frac{3}{\Delta_i}
        \end{split}
    \end{equation*}
\end{itemize}
To sum up, the total contribution of arm $i$ to the regret is at most (multiply by $Ck\log\frac{2n}{\delta}$)
\[R_i=(R_i^<+R_i^>)Ck\log\frac{2n}{\delta}\leq \bigg(\frac{2}{\Delta_i} + \frac{3}{\Delta_i}\bigg) Ck\log\frac{2n}{\delta}=O \bigg(\frac{1}{\Delta_i}k\log\frac{n}{\delta}\bigg)\]
\end{proof}

We now prove Theorem \ref{thm:regretUpperBound}.

\begin{proof}
The total regret of the algorithm is compounded of two parts. The first is the regret accumulated in the elimination process of the sub-optimal arms. Lemma \ref{lemma:individualArmRegret} provides a bound on the contribution of every sub-optimal arm to the regret, thus by summing over all sub-optimal arms we have

\[R_{sub}=\sum_{i=k+1}^n R_i\leq O\bigg(\sum_{i=k+1}^n \frac{1}{\Delta_i}k\log\frac{n}{\delta}\bigg)\]

The second part of the regret is the one accumulated in the process of estimating the top $2k$ arms. Since they are being estimated in each phase until the end of the run, that is until the arm with the minimal $\Delta$ is recognized, the number of times each one of them is sampled is proportional to $\frac{1}{\Delta^2}$. As they are the top $2k$ arms with high probability, the worst subset with regard to regret that can be sampled is the subset $\{k+1,\dots,2k\}$. The gap between this subset and the optimal subset is $\sum_{i=1}^k \Delta_{i:(k+i)}$ and thus the regret is bounded by 
\[R_{top}\leq\sum_{i=1}^k \frac{\Delta_{i:(k+i)}}{\Delta^2}Ck\log\frac{2n}{\delta}\]

In conclusion, the total regret of the algorithm is given by 
\[R=R_{sub}+R_{top}\leq O\Bigg(\bigg(\sum_{i=1}^k \frac{\Delta_{i:(k+i)}}{\Delta^2} + \sum_{i=k+1}^n \frac{1}{\Delta_i}\bigg) k\log\frac{n}{\delta}\Bigg)\]

Finally, we can translate it to terms of the time horizon $T$ by taking $\delta=\frac{1}{kT}$ similar to Theorem \ref{thm:weakRegret}.

\end{proof}


\begin{corollary}\label{thm:IndRegret}
The distribution-independent regret is at most
\begin{equation*}
    R= O\big(k\sqrt{nT\log T}\big)
\end{equation*}
\end{corollary}

\begin{proof}
For the distribution-independent upper bound, consider the $(\epsilon,\delta)$-PAC variant of CSAR (see Remark 3). Instead of running it until the last arm is recognized, we stop exploring when $\epsilon_t\leq\epsilon$. Then, we keep selecting the best $k$ estimated arms for the rest of the time horizon $T$. Note that when we stop, the arms estimations are at most $\epsilon$ far from their real expected value, according to Lemma \ref{lemma:PACest1}. Hence, the gap between the optimal subset and any subset of the arms that survived to phase $t$ is at most $k\epsilon$, and thus their regret is at most $R^<\leq k\epsilon T$. \\
This should be added to the regret caused by the arms that were eliminated up to this stage. According to Lemma \ref{lemma:individualArmRegret}, the contribution of a sub-optimal arm $i$ to the regret is bounded by $\frac{k}{\Delta_i}\log \frac{n}{\delta}$. Since it was eliminated before phase $t$, it must hold that $\Delta_i>\epsilon$. The number of eliminated arms is clearly bounded by $n$, and thus their contribution to the regret is
\[R^>\leq C\sum_{i:\Delta_i>\epsilon}\frac{k}{\Delta_i}\log T\leq C\sum_{i:\Delta_i>\epsilon}\frac{k}{\epsilon}\log T \leq C\frac{nk}{\epsilon}\log T\]
for some constant $C$. Concluding both parts of regret, we get
\[R\leq C\frac{nk}{\epsilon}\log T + \epsilon k T\]
This is true as long as the number of rounds is at least the number of samples done by CSAR up to phase $t$, that is $T\geq C'\frac{n}{\epsilon^2}\log \frac{n}{\delta}$ for some constant $C'$.
Thus for $\epsilon=\sqrt{\frac{C'n}{T}\log \frac{n}{\delta}}$ and $\delta=\frac{1}{kT}$ we get that the regret is bounded by
\[R=O\big(k\sqrt{nT\log T}\big)\]
\end{proof}


CSAR's distribution-independent regret is bigger by factor $\sqrt{k}$ than the $\Omega\big(\sqrt{knT}\big)$ lower bound in \cite{lattimore2018toprank} (ignoring $\log$ terms). In many cases it is reasonable to assume $k=O(1)$ which makes the bounds tight. As for the dependence on $k$, we leave the search for tighter bounds for further research. 

Assuming all gaps are equal to $\Delta$, the regret in (\ref{eqn:regret}) can be written as
$R= O\bigg(\frac{nk}{\Delta} \log T\bigg)$.
%To stress the necessity of the factor $k$ in the regret upper bound, 
We prove that it is tight for CSAR.


\begin{lemma}
For any $n,k$ and time horizon $T>n$, there exists a distribution over the assignment of rewards such that the regret of CSAR with EST2 is at least
\[R=\Omega\bigg(\frac{nk}{\Delta}\log T\bigg)\]
\end{lemma}

\begin{proof}
Consider the following example. Each arm $i\in [n]$ is associated with a Gaussian random variable $X_i\sim\mathcal{N}(\theta_i,1)$ where
\[\theta_i=\begin{cases}
\Delta & i\leq k\\
0 & i>k
\end{cases}\]
namely, for the optimal arms the expected reward is $\Delta$ and for the rest it is $0$. Similar to Lemma $\ref{lemma:armSampleComp}$, the best arms will be identified only when $\Delta>2\epsilon_t$ which implies that the number of phases is $T>\Omega(\log\frac{1}{\Delta})$, and since no arm is accepted or rejected until this phase the total number of samples is $\Omega\big(\frac{n}{\Delta^2}\log\frac{n}{\delta}\big)$. Additionally, each subset has a gap of up to $k\Delta$. Thus, the total regret is 
\[R=\Omega\big(k\Delta\cdot\frac{n}{\Delta^2}\log\frac{n}{\delta}\big)\]
which proves that the regret upper bound is tight.
\end{proof}


==> lower_bounds.tex <==
\section{Lower Bounds}
In this chapter we prove two lower bounds for combinatorial bandits with full-bandit feedback. The first bounds the minimal number of samples necessary to identify the best subset of $k$ arms, and the second bounds the regret that every algorithm must suffer as a function of the time horizon $T$.

\subsection{Sample Complexity}
One might wonder if the lower bound of $\Omega\big(\frac{n}{\epsilon^2}\log\frac{1}{\delta}\big)$ samples for best arm identification \cite{mannor2004sample} or $\Omega\big(\frac{n}{\epsilon^2}\log\frac{k}{\delta}\big)$ for multiple arms identification \cite{kaufmann2013information, kalyanakrishnan2012pac, chen2014combinatorial} applies also for combinatorial bandits. The answer is not immediate. Intuitively, sampling $k$ arms together might provide more information to the agent so that hypothetically it can use less samples to find the best set of arms. For example, if the goal is to detect an unknown number of counterfeit coins out of $n$ coins, and the agent is allowed to weigh any number of coins, then there exists an algorithm that identifies the counterfeit coins using only $\Theta\big(\frac{n}{\log n}\big)$ weighings, with or without the presence of noise \cite{erdos1963two,soderberg1963combinatory,bshouty2012coin}.
%Formally, since each sample is the sum of $k$ variables, it contains $\log k$ bits of information (up to the number of bits needed for representing each arm). Thus, if the lower bound for Explore-k is given by $\Omega(\frac{n}{\epsilon^2})$, a naive approach could expect to solve the combinatorial problem within $\Omega(\frac{n}{\epsilon^2\log k})$ samples.

% We demonstrate this intuition with an example. There are $n$ arms, each arm is associated with a constant number (instead of random variable), and the agent's objective is to find the best $k$. For simplicity, assume that there are $k$ arms with value $\epsilon$ and the rest are $0$s. The following algorithm finds the top $k$ using $O(\frac{n}{k}+k\log k)$ queries. First partition the arms into $\frac{n}{k}$ sets, query for each set and eliminate all the ones with outcome $0$. We are left with at most $k$ sets. In each of them, use binary search to find the hiding $\epsilon$s. This algorithm uses $\frac{n}{k}$ queries for the first step and $\log k$ queries for binary search in each of the $k$ sets. Thus the total number of queries is $O(\frac{n}{k}+k\log k)$ which is generally smaller than $\Omega(\frac{n}{\epsilon^2})$. However, this example assumed constant arms. It raises the question what is the case when the arms are random variables.

Despite the discussion above, the following theorem proves a lower bound of $\Omega\big(\frac{n}{\epsilon^2}\big)$ samples for combinatorial bandits, similar to the bounds for best- and multiple-arms identification tasks. This bound shows that CSAR is optimal with respect to sample complexity (up to $\log$ facotrs). 

\begin{theorem}\label{thm:lowerBound}
For any $n$ and $k\leq\frac{n}{2}$, and for any $0<\epsilon, \delta<\frac{1}{2}$, there exists a distribution over the assignment of rewards such that the sample complexity of any $(\epsilon,\delta)$-PAC algorithm is at least
\[M=\Omega\Big(\frac{n}{\epsilon^2}\Big)\]
\end{theorem}

The proof is based on \citet[chap.~2]{slivkins2019introduction}, but generalized for the combinatorial setting.  It defines two problem instances with small KL-divergence between them and shows that any algorithm that uses less samples than required is wrong with high probability.

\input{lower_bound_proof.tex}

\newpage
\subsection{Regret}
As mentioned in Section \ref{sc:relatedWork}, the existing lower bound of $\Omega\big(k\sqrt{nT}\big)$ for full-bandit \cite{audibert2013regret} assumes constraints on the subset selection, which is not the case in our setting. Instead, only a weaker lower bound of $\Omega\big(\sqrt{knT}\big)$ that was proven for semi-bandit \cite{lattimore2018toprank} applies to our setting.

As a supplement, we present some alternative proofs that use some slightly different techniques.
We begin with a weaker bound of $\Omega\big(\sqrt{nT}\big)$ that follows from the sample complexity bound, and then prove a stronger $\Omega\big(\sqrt{knT}\big)$ bound, equivalent to the one in \cite{lattimore2018toprank}.

\subsubsection{Lower bound of $\Omega(\sqrt{nT})$}
\begin{theorem}\label{thm:lowerBoundRegret}
For any $n$ and $k\leq\frac{n}{2}$, and for any time horizon $T>n$, there exists a distribution of rewards such that the expected regret of any algorithm is at least
\[R=\Omega\big(\sqrt{nT}\big)\]
\end{theorem}

\begin{proof}
We use the lower bound on sample complexity in Theorem \ref{thm:lowerBound} to prove a lower bound on the regret. For any round $t\in[T]$ define
\[B_t=\{j\in[n]\,|\,Pr[j\in S_t|\mathcal{I}_j]\leq\frac{3}{4}\}\]
By (\ref{eqn:BsetProbs}) for any $t$, $B_t\geq\frac{n}{3}$.
Consider a uniform distribution over the profiles instances $\mathcal{I}_j$. In what follows, the expectations are over the choice of $\mathcal{I}_j$ as well as the random rewards and the randomness in the algorithm.
Since $\mathcal{I}_j$ have mean reward $\mu^*=\frac{k}{2}+\epsilon$ on any subset $S$ that contains $j$, and mean reward $\frac{k}{2}$ on the other subsets, we have
\begin{equation*}
\begin{split}
    \mathbb{E}[\mu(S_t)|j\in B_t]=&\frac{k}{2}Pr[j\notin S_t|j\in B_t]+\Big(\frac{k}{2}+\epsilon\Big)Pr[j\in S_t|j\in B_t]\\
    =&\frac{k}{2}+\epsilon Pr[j\in S_t|j\in B_t]\leq\frac{k}{2}+\frac{3}{4}\epsilon
\end{split}
\end{equation*}

Therefore for all $t$, $\mathbb{E}[\Delta_t|j\in B_t]\geq{1}{4}\epsilon$ and the expected regret is
\begin{equation*}
\begin{split}
\mathbb{E}[\Delta_t]\geq\mathbb{E}[\Delta_t|j\in B_t]Pr[j\in B_t]\geq\frac{1}{4}\epsilon\cdot\frac{1}{3}=\frac{1}{12}\epsilon
\end{split}
\end{equation*}
and finally $\mathbb{E}[R]=\sum_{t=1}^T \mathbb{E}[\Delta_t]\geq\frac{1}{12}\epsilon T$, where we assumed $T\leq\frac{cn}{\epsilon^2}$. Taking $\epsilon=\sqrt{\frac{cn}{T}}$ gives the desired lower bound on the regret
\[R\geq\Omega\big(\sqrt{nT}\big)\]
\end{proof}

\subsubsection{Lower bound of $\Omega(\sqrt{knT})$}
We now prove a stronger lower bound, similar to the one in \cite{lattimore2018toprank} and also \cite{auer2002nonstochastic,cesa2006prediction}.
\begin{theorem}\label{thm:bestLowerBoundRegret}
For any $n$ and $k\leq\sqrt{n}$, and for any time horizon $T>n$, there exists a distribution of rewards such that the expected regret of any algorithm is at least
\[R=\Omega\big(\sqrt{knT}\big)\]
\end{theorem}

Define the following profiles: for each $S\subset[n], |S|=k$ we define the following profile
\[\mathcal{I}_S=
\begin{cases}
X_i\sim \mathcal{N}(\frac{\epsilon}{k},1) & i\in S\\
X_i\sim \mathcal{N}(0,1) & i\notin S
\end{cases}\]
We also define $\mathcal{I}_0=\{X_i\sim \mathcal{N}(0,1)\,|\,i=1\dots n\}$.

For any profile $\mathcal{I}_S$ and a sequence of subsets $S_1\dots S_T$ taken by the agent, denote by $X_{S}^t=|S_t\cap S|$ the size of the intersection between the subset $S_t$ selected by the agent at step $t$ and the optimal subset $S$. In other words, $X_{S}^t$ is the number of optimal arms taken by the agent at step $t$.

We first bound the KL divergence between the probability distribution observed by the agent given profile $\mathcal{I}_S$ and $\mathcal{I}_0$.

\begin{lemma}
Let $P_S^T$ ($P_0^T$) be the probability distribution observed by the agent over $T$ steps given profile $\mathcal{I}_S$ ($\mathcal{I}_0$ accordingly), then
\[KL(P_S,P_0)=\frac{\epsilon^2}{k^3}\sum_{t=1}^T \mathbb{E}\big[(X_S^t)^2\,\big|\,\mathcal{I}_0\big]\]
\end{lemma}
\begin{proof}
For any profile $\mathcal{I}_S$ and any subset $S_t$ taken by the agent at step $t$, denote by $Y_S^t$ the random variable of aggregated reward observed by the agent. Recall that the KL divergence between two gaussians with variance $\sigma^2$ and means $\mu_1$ and $\mu_2$ is given by $\frac{(\mu_1-\mu_2)^2}{\sigma^2}$. Hence, assume that $X_S^t=i$ for some $i=1\dots k$ then
\[KL(Y_S^t,Y_0^t)=\frac{(i\times \frac{\epsilon}{k})^2}{k}=i^2\frac{\epsilon^2}{k^3}\]
Accordingly we can bound the divergence between $P_S$ and $P_0$ by
\[KL(P_S,P_0)=\sum_{t=1}^T KL(Y_S^{t},Y_0^{t})=\sum_{t=1}^T\sum_{i=1}^{k} Pr[X_S^t=i\,|\,\mathcal{I}_0] i^2\frac{\epsilon^2}{k^3}=\frac{\epsilon^2}{k^3}\sum_{t=1}^T \mathbb{E}\big[(X_S^t)^2\,\big|\,\mathcal{I}_0\big]
\]
\end{proof}

\begin{corollary}\label{cor:regretBound}
By Pinsker's inequality, for any function $f:\mathbb{R}^{T}\mapsto [0,M]$ defined on reward sequence $\textbf{r}\in\mathbb{R}^T$,
\begin{equation*}
    \begin{split}
        \mathbb{E}[f(\textbf{r})\,|\,\mathcal{I}_S] - \mathbb{E}[f(\textbf{r})\,|\,\mathcal{I}_0] \leq M \norm{P_S-P_0}_1\leq 
        M \sqrt{2KL(P_S,P_0)}=M\sqrt{\frac{2\epsilon^2}{k^3}\sum_{t=1}^T \mathbb{E}[(X_S^t)^2|\mathcal{I}_0]}
    \end{split}
\end{equation*}
\end{corollary}

We now prove Theorem \ref{thm:bestLowerBoundRegret}.
\begin{proof}
Fix an agent and a profile $\mathcal{I}_S$, and let $f(\textbf{r})=\sum_{t=1}^T X_S^t$, then the maximal value of $F$ is $kT$ and thus by Corollary \ref{cor:regretBound},
\begin{equation}\label{eq:advantage}
    \mathbb{E}\Big[\sum_{t=1}^T X_S^t \,\Big|\, \mathcal{I}_S\Big] - \mathbb{E}\Big[\sum_{t=1}^T X_S^t\,\Big|\,\mathcal{I}_0\Big] \leq kT \sqrt{\frac{2\epsilon^2}{k^3}\sum_{t=1}^T \mathbb{E}\big[(X_S^t)^2\,\big|\,\mathcal{I}_0\big]}
\end{equation}

Assuming that the profile is chosen uniformly over all $\binom{n}{k}$ subsets, we average (\ref{eq:advantage}) over the subsets. Note that if $S$ is chosen randomly, then under the profile $\mathcal{I}_0$, for any $t$ $X_S^{t}$ is a hypergeometric variable with population size $n$, $k$ draws and $k$ successes. Then its' expected value is $\frac{k^2}{n}$. Accordingly,
\[\mathbb{E}_{S}\bigg[\mathbb{E}\Big[\sum_{t=1}^T X_S^t\,\Big|\,\mathcal{I}_0\Big]\bigg]= \sum_{t=1}^T \mathbb{E}_{S}\Big[\mathbb{E}\big[ X_S^t\,\big|\,\mathcal{I}_0\big]\Big]=\sum_{t=1}^T\frac{k^2}{n}=T\frac{k^2}{n}\]
and in the right hand side of (\ref{eq:advantage}) we use Jensen inequality to get
\[\mathbb{E}_{S}\bigg[\sqrt{\sum_{t=1}^T \mathbb{E}\big[(X_S^t)^2\,\big|\,\mathcal{I}_0\big]}\bigg]\leq \sqrt{\sum_{t=1}^T \mathbb{E}_{S}\Big[\mathbb{E}\big[(X_S^t)^2\,\big|\,\mathcal{I}_0\big]\Big]}\leq \sqrt{2\frac{k^2}{n}T}\]
where we used the fact that for the hypergeometric variable $X_S^t$ it holds $\mathbb{E}\big[(X_S^t)^2\big]\leq 2\frac{k^2}{n}$ for $k\leq\sqrt{n}$.
Substituting in (\ref{eq:advantage}) we have

\[\mathbb{E}_{S}\bigg[\mathbb{E}\Big[\sum_{t=1}^T X_S^t \,\Big|\, \mathcal{I}_S\Big]\bigg] \leq T\frac{k^2}{n} + kT\sqrt{\frac{2\epsilon^2}{k^3}\frac{2k^2}{n}T}=T\frac{k^2}{n} + 2\epsilon T\sqrt{\frac{T}{kn}}\]

Fix a profile $\mathcal{I}_S$. To bound the regret, note that the optimal expected reward is $\epsilon$ while the expected reward of the subset taken by the agent at step $t$ is $X_S^t\frac{\epsilon}{k}$, thus expected regret is by definition
\[R=\sum_{t=1}^T \epsilon - X_S^t\frac{\epsilon}{k}\]
Accordingly, if the profile $\mathcal{I}_S$ is selected randomly over all subsets, then the regret is
\[\begin{split}
    \mathbb{E}_S[R]=& \epsilon T - \frac{\epsilon}{k}\mathbb{E}_S\Big[\sum_{t=1}^T X_S^t\,\Big|\,\mathcal{I}_S\Big] \geq \epsilon T - \frac{\epsilon}{k}\Big(T\frac{k^2}{n} + 2\epsilon T\sqrt{\frac{T}{kn}}\Big)\geq \\ 
    \geq &\epsilon T\Big(1-\frac{k}{n}-2\epsilon\sqrt{\frac{T}{kn}}\Big)\geq \epsilon T\Big(\frac{1}{2}-2\epsilon\sqrt{\frac{T}{kn}}\Big)
\end{split}\]
where we assumed $k\leq\frac{n}{2}$. \\
This is true for any $\epsilon$, thus for $\epsilon=\frac{1}{8}\sqrt{\frac{kn}{T}}$ we have
\[\mathbb{E}_S[R]\geq\frac{1}{4}\sqrt{knT}\]
as desired
\end{proof}

%Note that for CSAR we proved a regret upper bound of $O(k\sqrt{nT})$, which is bigger by a factor of $\sqrt{k}$. However, assuming $k=O(1)$ the bounds are tight, meaning that CSAR is optimal.
%meaning that either CSAR is not optimal or there is a stronger lower bound. We conjecture that the latter is true, and that the lower bound on regret must depend on $k$, since the subsets consist of $k$ arms and thus the gap between the optimal subset and the subset taken by the agent in each round is of order of $k$.

